Muffin: Testing Deep Learning Libraries via Neural Architecture Fuzzing

Deep learning (DL) techniques are proven effective in many challenging tasks, and become widely-adopted in practice. However, previous work has shown that DL libraries, the basis of building and executing DL models, contain bugs and can cause severe consequences. Unfortunately, existing testing approaches still cannot comprehensively exercise DL libraries. They utilize existing trained models and only detect bugs in model inference phase. In this work we propose Muffin to address these issues. To this end, Muffin applies a specifically-designed model fuzzing approach, which allows it to generate diverse DL models to explore the target library, instead of relying only on existing trained models. Muffin makes differential testing feasible in the model training phase by tailoring a set of metrics to measure the inconsistencies between different DL libraries. In this way, Muffin can best exercise the library code to detect more bugs. To evaluate the effectiveness of Muffin, we conduct experiments on three widely-used DL libraries. The results demonstrate that Muffin can detect 39 new bugs in the latest release versions of popular DL libraries, including Tensorflow, CNTK, and Theano.

==> figures/other_figures/KCI_per.tex <==
  \begin{tikzpicture}[font=\small]
    \begin{axis}[
      ybar,
      bar width=21pt,
      xlabel={Quality},
      ylabel={Probability},
      ymin=0,
      ymax=100,
      ytick=\empty,
      xtick=data,
      axis x line=bottom,
      axis y line=left,
      enlarge x limits=0.2,
      symbolic x coords={S1, S2, S3, S4,S5,S6,S7},
      xticklabel style={anchor=base,yshift=-\baselineskip},
      nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%}
    ]
      \addplot[fill=white] coordinates {
        (S1,68.83)
        (S2,73.6)
        (S3,85.88)
        (S4,75.8)
        (S5,75.82)
        (S6,93.44)
        (S7,70.52)
      };
    \end{axis}
  \end{tikzpicture}

==> tables/incons_all.tex <==
\begin{table*}[t!]
    \centering
    \caption{Comparison of inconsistency number}
    \renewcommand{\arraystretch}{0.7}
    \resizebox{0.85\textwidth}{!}{
        \begin{threeparttable}

        \begin{tabular}{@{}l|l|l|ccc|ccc|ccc|ccc|ccc|ccc|ccc@{}}
            \toprule
            \multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Method}}   & \multirow{2}{*}{\textbf{Lib Pair}} & \multicolumn{3}{c|}{\textbf{CIFAR-10}}  & \multicolumn{3}{c|}{\textbf{MNIST}}     & \multicolumn{3}{c|}{\textbf{F-MNIST}} & \multicolumn{3}{c|}{\textbf{ImageNet}}  & \multicolumn{3}{c|}{\textbf{Sine-Wave}} & \multicolumn{3}{c|}{\textbf{Stock-Price}} & \multicolumn{3}{c}{\textbf{Total}}     \\
                                            &                                    &                                    & \textbf{FC} & \textbf{LC} & \textbf{BC} & \textbf{FC} & \textbf{LC} & \textbf{BC} & \textbf{FC}   & \textbf{LC}  & \textbf{BC}  & \textbf{FC} & \textbf{LC} & \textbf{BC} & \textbf{FC} & \textbf{LC} & \textbf{BC} & \textbf{FC}  & \textbf{LC}  & \textbf{BC} & \textbf{FC} & \textbf{LC} & \textbf{BC} \\ \midrule
            \multirow{9}{*}{\textbf{E1}}    & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF-TH}                     &4             &0             &0             &4             &0             &0             &7               &1              &1              &1             &1             &0             &5              &0             &0             &3              &1              &0             &16             &2             &1             \\
                                            &                                    & \textbf{TF-CK}                     &3             &1             &0             &4             &2             &1             &6               &2              &1              &3             &1             &0             &12             &0             &0             &8              &0              &0             &16             &2             &2             \\
                                            &                                    & \textbf{TH-CK}                     &4             &1             &0             &4             &0             &0             &7               &1              &1              &1             &0             &0             &6              &0             &0             &2              &0              &0             &13             &1             &1             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{LEMON}}    & \textbf{TF-TH}                     &1             &-             &-             &0             &-             &-             &1               &-              &-              &1             &-             &-             &0             &-             &-             &0              &-              &-             &2             &-             &-             \\
                                            &                                    & \textbf{TF-CK}                     &1             &-             &-             &0             &-             &-             &0               &-              &-              &1             &-             &-             &1             &-             &-             &0              &-              &-             &3             &-             &-             \\
                                            &                                    & \textbf{TH-CK}                     &0             &-             &-             &0             &-             &-             &1               &-              &-              &0             &-             &-             &1             &-             &-             &0              &-              &-             &2             &-             &-             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{\base}} & \textbf{TF-TH}                     &1             &0             &3             &4             &2             &2             &2               &0              &2              &5             &0             &0             &1             &0             &0             &0              &1              &0             &9             &2             &3             \\
                                            &                                    & \textbf{TF-CK}                     &2             &1             &1             &1             &2             &1             &1               &3              &1              &2             &2             &0             &2             &0             &0             &4              &1              &0             &5             &3             &1             \\
                                            &                                    & \textbf{TH-CK}                     &1             &0             &0             &3             &1             &1             &2               &0              &1              &5             &0             &0             &2             &0             &0             &4              &0              &0             &10            &1             &1             \\ \midrule
            \multirow{9}{*}{\textbf{E2}}    & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF-TH}                     &7             &0             &1             &5             &0             &1             &8               &1              &0              &3             &1             &1              &6             &0             &0             &1              &0              &0             &16             &1             &2             \\
                                            &                                    & \textbf{TF-CK}                     &7             &2             &0             &4             &2             &0             &6               &2              &0              &6             &1             &0              &6             &0             &0             &7              &0              &0             &20             &2             &0             \\
                                            &                                    & \textbf{TH-CK}                     &8             &1             &1             &5             &1             &0             &8               &1              &0              &3             &0             &1              &6             &0             &0             &2              &0              &0             &16             &1             &1             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{LEMON}}    & \textbf{TF-TH}                     &1             &-             &-             &0             &-             &-             &1               &-              &-              &1             &-             &-             &0             &-             &-             &0              &-              &-             &2             &-             &-             \\
                                            &                                    & \textbf{TF-CK}                     &1             &-             &-             &0             &-             &-             &0               &-              &-              &1             &-             &-             &1             &-             &-             &0              &-              &-             &3             &-             &-             \\
                                            &                                    & \textbf{TH-CK}                     &0             &-             &-             &0             &-             &-             &1               &-              &-              &0             &-             &-             &1             &-             &-             &0              &-              &-             &2             &-             &-             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{\base}} & \textbf{TF-TH}                     &2             &1             &1             &3             &0             &1             &2               &1              &3              &4             &1             &1             &4             &0             &0             &0              &0              &0             &9              &2             &4             \\
                                            &                                    & \textbf{TF-CK}                     &3             &2             &2             &1             &1             &1             &2               &2              &3              &2             &2             &1             &4             &0             &0             &2              &0              &0             &8              &2             &4             \\
                                            &                                    & \textbf{TH-CK}                     &4             &0             &0             &4             &0             &0             &2               &0              &2              &5             &1             &0             &5             &0             &0             &1              &0              &0             &10             &1             &2             \\ \midrule
            \multirow{9}{*}{\textbf{E3}}    & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF-TH}                     &4             &0             &0             &2             &0             &0             &5               &1              &1              &3             &0             &0             &1             &0             &0             &1              &0              &0             &11             &1             &1             \\
                                            &                                    & \textbf{TF-CK}                     &3             &0             &1             &8             &0             &0             &6               &1              &1              &8             &0             &1             &5             &0             &0             &6              &0              &0             &17             &1             &3             \\
                                            &                                    & \textbf{TH-CK}                     &3             &0             &0             &4             &1             &0             &5               &1              &0              &5             &0             &0             &2             &0             &0             &6              &0              &0             &13             &1             &0             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{LEMON}}    & \textbf{TF-TH}                     &1             &-             &-             &0             &-             &-             &1               &-              &-              &1             &-             &-             &0             &-             &-             &0              &-              &-             &2             &-             &-             \\
                                            &                                    & \textbf{TF-CK}                     &1             &-             &-             &0             &-             &-             &0               &-              &-              &1             &-             &-             &1             &-             &-             &0              &-              &-             &3             &-             &-             \\
                                            &                                    & \textbf{TH-CK}                     &0             &-             &-             &0             &-             &-             &1               &-              &-              &0             &-             &-             &1             &-             &-             &0              &-              &-             &2             &-             &-             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{\base}} & \textbf{TF-TH}                     &5             &0             &1             &4             &0             &1             &3               &1              &2              &3             &0             &2             &2             &0             &0             &0              &0              &0             &8              &1             &3             \\
                                            &                                    & \textbf{TF-CK}                     &4             &0             &1             &4             &2             &2             &2               &1              &2              &3             &2             &1             &2             &0             &0             &2              &0              &0             &9              &4             &3             \\
                                            &                                    & \textbf{TH-CK}                     &6             &0             &1             &5             &0             &0             &4               &1              &0              &4             &1             &0             &3             &0             &0             &2              &0              &0             &10             &1             &1             \\ \midrule
            \multirow{9}{*}{\textbf{E4}}    & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF-TH}                     &4             &0             &0             &3             &0             &1             &4               &0              &0              &1             &0             &0             &1             &0             &0             &0              &0              &0             &9              &0             &1             \\
                                            &                                    & \textbf{TF-CK}                     &7             &1             &1             &4             &1             &1             &4               &1              &1              &4             &0             &0             &4             &0             &0             &2              &0              &0             &11             &1             &2             \\
                                            &                                    & \textbf{TH-CK}                     &5             &0             &0             &4             &0             &0             &4               &0              &0              &1             &0             &0             &2             &0             &0             &0              &0              &0             &11             &0             &0             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{LEMON}}    & \textbf{TF-TH}                     &1             &-             &-             &0             &-             &-             &1               &-              &-              &1             &-             &-             &0             &-             &-             &0              &-              &-             &2             &-             &-             \\
                                            &                                    & \textbf{TF-CK}                     &1             &-             &-             &0             &-             &-             &0               &-              &-              &1             &-             &-             &1             &-             &-             &0              &-              &-             &3             &-             &-             \\
                                            &                                    & \textbf{TH-CK}                     &0             &-             &-             &0             &-             &-             &1               &-              &-              &0             &-             &-             &1             &-             &-             &0              &-              &-             &2             &-             &-             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{\base}} & \textbf{TF-TH}                     &7             &1             &2             &2             &0             &1             &4               &1              &2              &4             &0             &1             &1             &0             &0             &0              &0              &0             &8              &1             &3             \\
                                            &                                    & \textbf{TF-CK}                     &3             &1             &0             &4             &0             &1             &2               &1              &1              &3             &2             &1             &2             &0             &0             &4              &0              &0             &7              &2             &1             \\
                                            &                                    & \textbf{TH-CK}                     &7             &1             &1             &4             &0             &0             &5               &1              &2              &5             &0             &0             &2             &0             &0             &4              &0              &0             &10             &1             &2             \\ \midrule
            \multirow{9}{*}{\textbf{E5}}    & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF-TH}                     &6             &0             &0             &6             &0             &0             &5               &0              &1              &4             &0             &1             &2             &0             &0             &4              &0              &0             &11             &0             &1             \\
                                            &                                    & \textbf{TF-CK}                     &1             &1             &0             &4             &1             &0             &1               &1              &1              &1             &0             &0             &3             &0             &0             &4              &0              &0             &7             &1             &1             \\
                                            &                                    & \textbf{TH-CK}                     &3             &1             &0             &4             &0             &0             &5               &1              &0              &2             &0             &1             &4             &0             &0             &5              &0              &0             &9             &1             &1             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{LEMON}}    & \textbf{TF-TH}                     &1             &-             &-             &0             &-             &-             &1               &-              &-              &0             &-             &-             &0             &-             &-             &0              &-              &-             &1             &-             &-             \\
                                            &                                    & \textbf{TF-CK}                     &1             &-             &-             &0             &-             &-             &0               &-              &-              &0             &-             &-             &1             &-             &-             &0              &-              &-             &2             &-             &-             \\
                                            &                                    & \textbf{TH-CK}                     &0             &-             &-             &0             &-             &-             &1               &-              &-              &0             &-             &-             &1             &-             &-             &0              &-              &-             &2             &-             &-             \\ \cmidrule(l){2-24} 
                                            & \multirow{3}{*}{\textbf{\base}} & \textbf{TF-TH}                     &4             &0             &2             &3             &0             &2             &3               &0              &1              &2             &0             &0             &4             &0             &0             &0              &0              &0             &11              &0             &3             \\
                                            &                                    & \textbf{TF-CK}                     &4             &1             &1             &3             &0             &3             &4               &0              &1              &1             &0             &0             &3             &0             &0             &3              &0              &0             &9              &1             &3             \\
                                            &                                    & \textbf{TH-CK}                     &2             &1             &0             &3             &1             &1             &5               &0              &0              &3             &0             &0             &6             &0             &0             &3              &0              &0             &12             &2             &1             \\ \bottomrule
        \end{tabular}

        % 表格注释
        \begin{tablenotes}
            \footnotesize
            \item[1] "TF-TH""TF-CK" and "TH-CK" are respectively short for library pair "TensorFlow-Theano""TensorFlow-CNTK" and "Theano-CNTK".
            \item[2] "FC""LC""BC" respectively represent the number of layer inconsistencies(or loss inconsistencies) detected in the three stages. For inconsistencies caused by the same kind of layer(or loss function), we only count once.
        \end{tablenotes}

        \end{threeparttable}
    }
  \label{table:incons}
\end{table*}



==> tables/nan_crash_all.tex <==
\begin{table*}[t!]
    \centering
    \caption{Comparison of NaN/crash number}
    \renewcommand{\arraystretch}{0.7}
    \resizebox{0.9\textwidth}{!}{
     \begin{threeparttable}

        \begin{tabular}{@{}l|l|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc@{}}
            \toprule
            \multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Method}}   & \multirow{2}{*}{\textbf{Lib}} & \multicolumn{3}{c|}{\textbf{CIFAR-10}} & \multicolumn{3}{c|}{\textbf{MNIST}} & \multicolumn{3}{c|}{\textbf{F-MNIST}} & \multicolumn{3}{c|}{\textbf{ImageNet}} & \multicolumn{3}{c|}{\textbf{Sine-Wave}} & \multicolumn{3}{c|}{\textbf{Stock-Price}} & \multicolumn{3}{c}{\textbf{Total}} \\
                                         &                                    &                            & \textbf{NaN}      & \textbf{MGC}  & \textbf{IDC}     & \textbf{NaN}    & \textbf{MGC}  & \textbf{IDC}    & \textbf{NaN}        & \textbf{MGC}  & \textbf{IDC}        & \textbf{NaN}      & \textbf{MGC}  & \textbf{IDC}     & \textbf{NaN}      & \textbf{MGC}  & \textbf{IDC}      & \textbf{NaN}       & \textbf{MGC}  & \textbf{IDC}       & \textbf{NaN}    & \textbf{MGC}  & \textbf{IDC}    \\ \midrule
            \multirow{9}{*}{\textbf{E1}} & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF}           &2                   &0  &1                 &3                 &0 &1                 &3                     &0 &1                     &5                   &0 &1                  &4                   &0 &1                   &5                    &0 &1                    &7                 &0 &1                    \\
                                         &                                    & \textbf{TH}           &3                   &0  &10                &2                 &0 &10                &1                     &0 &3                     &2                   &0 &3                  &3                   &0 &8                   &3                    &0 &4                    &6                 &0 &10                   \\
                                         &                                    & \textbf{CK}           &2                   &6  &4                 &3                 &6 &4                 &3                     &4 &3                     &4                   &2 &2                  &4                   &4 &4                   &5                    &4 &4                    &7                 &6 &4                    \\ \cmidrule(l){2-24} 
                                         & \textbf{LEMON}                     & \textbf{-}            &0                   &-  &0                 &0                 &-  &0                &0                     &-  &0                    &0                   &-  &0                 &0                   &-  &0                  &0                    &-  &0                   &0                 &-  &0                \\ \cmidrule(l){2-24} 
                                         & \multirow{3}{*}{\textbf{\base}} & \textbf{TF}           &0                   &0  &0                 &0                 &0  &0                &0                     &0  &0                    &0                   &0  &0                 &4                   &0  &0                  &0                    &0  &0                   &4                 &0  &0                \\
                                         &                                    & \textbf{TH}           &0                   &0  &3                 &0                 &0  &3                &0                     &0  &2                    &0                   &0  &2                 &4                   &0  &3                  &0                    &0  &3                   &4                 &0  &3                \\
                                         &                                    & \textbf{CK}           &0                   &1  &4                 &0                 &0  &4                &0                     &0  &3                    &0                   &0  &2                 &5                   &0  &4                  &0                    &0  &3                   &5                 &1  &4                \\ \midrule
            \multirow{9}{*}{\textbf{E2}} & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF}           &4                   &1  &1                 &2                 &1  &1                &3                     &1  &1                    &2                   &0  &1                 &7                   &1  &1                  &4                    &1  &1                   &7                 &1  &1                \\
                                         &                                    & \textbf{TH}           &3                   &0  &5                 &1                 &0  &4                &3                     &0  &3                    &2                   &0  &3                 &5                   &0  &4                  &3                    &0  &4                   &7                 &0  &5                \\
                                         &                                    & \textbf{CK}           &2                   &3  &4                 &3                 &3  &4                &2                     &2  &3                    &2                   &0  &3                 &6                   &2  &4                  &4                    &2  &4                   &7                 &3  &4                \\ \cmidrule(l){2-24} 
                                         & \textbf{LEMON}                     & \textbf{-}            &0                   &-  &0                 &0                 &-  &0                &0                     &-  &0                    &0                   &-  &0                 &0                   &-  &0                  &0                    &-  &0                   &0                 &-  &0                \\ \cmidrule(l){2-24} 
                                         & \multirow{3}{*}{\textbf{\base}} & \textbf{TF}           &0                   &0  &0                 &0                 &0  &0                &1                     &0  &0                    &1                   &0  &0                 &3                   &0  &0                  &0                    &0  &0                   &4                 &0  &0                \\
                                         &                                    & \textbf{TH}           &0                   &0  &4                 &0                 &0  &4                &1                     &0  &4                    &1                   &0  &3                 &4                   &0  &4                  &0                    &0  &4                   &5                 &0  &4                \\
                                         &                                    & \textbf{CK}           &0                   &0  &4                 &0                 &0  &3                &1                     &0  &1                    &1                   &0  &1                 &3                   &0  &3                  &0                    &0  &3                   &4                 &0  &4                \\ \midrule
            \multirow{9}{*}{\textbf{E3}} & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF}           &2                   &6  &1                 &5                 &6  &1                &3                     &5  &1                    &3                   &2  &1                 &3                   &5  &1                  &3                    &5  &1                   &8                 &6  &1                \\
                                         &                                    & \textbf{TH}           &2                   &2  &9                 &5                 &2  &7                &3                     &2  &5                    &1                   &1  &5                 &1                   &2  &7                  &1                    &2  &5                   &8                 &2  &9                \\
                                         &                                    & \textbf{CK}           &2                   &6  &2                 &5                 &5  &2                &4                     &4  &2                    &3                   &2  &2                 &3                   &5  &2                  &3                    &4  &2                   &9                 &6  &2                \\ \cmidrule(l){2-24} 
                                         & \textbf{LEMON}                     & \textbf{-}            &0                   &-  &1                 &0                 &-  &0                &0                     &-  &0                    &0                   &-  &0                 &0                   &-  &0                  &0                    &-  &0                   &0                 &-  &1                \\ \cmidrule(l){2-24} 
                                         & \multirow{3}{*}{\textbf{\base}} & \textbf{TF}           &0                   &2  &1                 &0                 &2  &1                &1                     &1  &1                    &0                   &1  &1                 &3                   &2  &1                  &0                    &2  &1                   &4                 &2  &1                \\
                                         &                                    & \textbf{TH}           &0                   &1  &6                 &0                 &1  &6                &1                     &0  &3                    &0                   &0  &4                 &3                   &1  &6                  &0                    &1  &5                   &4                 &1  &6                \\
                                         &                                    & \textbf{CK}           &0                   &2  &2                 &0                 &2  &2                &1                     &1  &2                    &0                   &1  &2                 &3                   &2  &2                  &0                    &2  &2                   &4                 &2  &2                \\ \midrule
            \multirow{9}{*}{\textbf{E4}} & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF}           &1                   &9  &1                 &5                 &9  &1                &4                     &8  &1                    &3                   &5  &1                 &5                   &9  &1                  &2                    &7  &1                   &8                 &9  &1                \\
                                         &                                    & \textbf{TH}           &1                   &2  &9                 &2                 &2  &8                &1                     &2  &7                    &1                   &1  &6                 &3                   &2  &7                  &3                    &2  &7                   &6                 &2  &9                \\
                                         &                                    & \textbf{CK}           &1                   &4  &2                 &4                 &4  &2                &3                     &4  &2                    &3                   &3  &2                 &4                   &4  &2                  &4                    &4  &2                   &8                 &4  &2                \\ \cmidrule(l){2-24} 
                                         & \textbf{LEMON}                     & \textbf{-}            &0                   &-  &3                 &0                 &-  &0                &0                     &-  &0                    &0                   &-  &0                 &0                   &-  &0                  &0                    &-  &0                   &0                 &-  &3                \\ \cmidrule(l){2-24} 
                                         & \multirow{3}{*}{\textbf{\base}} & \textbf{TF}           &0                   &2  &1                 &1                 &2  &1                &0                     &1  &1                    &0                   &1  &1                 &3                   &2  &1                  &0                    &2  &1                   &4                 &2  &1                \\
                                         &                                    & \textbf{TH}           &0                   &1  &6                 &1                 &1  &5                &0                     &0  &4                    &0                   &0  &2                 &3                   &1  &5                  &0                    &1  &4                   &4                 &1  &6                \\
                                         &                                    & \textbf{CK}           &0                   &3  &2                 &1                 &3  &2                &0                     &2  &2                    &0                   &1  &1                 &3                   &3  &2                  &0                    &3  &2                   &4                 &3  &2                \\ \midrule
            \multirow{9}{*}{\textbf{E5}} & \multirow{3}{*}{\textbf{RMG}}      & \textbf{TF}           &4                   &5  &1                 &2                 &6  &1                &2                     &2  &1                    &5                   &2  &1                 &4                   &6  &1                  &2                    &3  &1                   &7                 &6  &1                \\
                                         &                                    & \textbf{TH}           &4                   &2  &9                 &2                 &2  &9                &2                     &1  &7                    &4                   &0  &5                 &2                   &2  &7                  &3                    &2  &7                   &5                 &2  &9                 \\
                                         &                                    & \textbf{CK}           &1                   &5  &3                 &3                 &4  &3                &2                     &2  &1                    &4                   &2  &1                 &3                   &4  &3                  &3                    &3  &3                   &7                 &5  &3                \\ \cmidrule(l){2-24} 
                                         & \textbf{LEMON}                     & \textbf{-}            &0                   &-  &1                 &0                 &-  &0                &0                     &-  &0                    &0                   &-  &2                 &0                   &-  &0                  &0                    &-  &0                   &0                 &-  &3                \\ \cmidrule(l){2-24} 
                                         & \multirow{3}{*}{\textbf{\base}} & \textbf{TF}           &1                   &2  &1                 &0                 &2  &1                &0                     &0  &1                    &0                   &0  &1                 &2                   &1  &1                  &0                    &1  &1                   &3                 &2  &1                \\
                                         &                                    & \textbf{TH}           &1                   &1  &4                 &0                 &1  &4                &0                     &0  &2                    &0                   &0  &2                 &2                   &1  &4                  &0                    &1  &3                   &3                 &1  &4                \\
                                         &                                    & \textbf{CK}           &1                   &3  &3                 &0                 &3  &2                &0                     &1  &2                    &0                   &1  &1                 &2                   &2  &2                  &0                    &2  &2                   &3                 &3  &3                \\ \midrule

            \end{tabular}

        % 表格注释
        \begin{tablenotes}
            \footnotesize
            \item[1] "TF""TH" and "CK" are respectively short for library name "TensorFlow""Theano" and "CNTK".
            \item[2] "NaN" represents the number of outputs with NaN. For NaN caused by the same kind of layer, we only count once.
            \item[3] "MGC" and "IDC" are respectively short for "Model Generation Crash" and "Inconsistency Detection Crash". The crash number have been deduplicated by the error messages.
            \item[4] Since LEMON does not record NaN/crash information for each backend, we only obtain the total NaN/crash number triggered by LEMON.
        \end{tablenotes}

    \end{threeparttable}
    }
    \label{table:nan_crash}
\end{table*}


==> tables/run_lemon_models.tex <==
\begin{table}[t!]
    \centering
    \caption{Additional experiment between RMG and LEMON using existing model under E1}
    \renewcommand{\arraystretch}{0.7}
    \resizebox{0.9\linewidth}{!}{
     \begin{threeparttable}

        \begin{tabular}{@{}l|l|ccc|ccc@{}}
            \toprule
            \multirow{2}{*}{\textbf{Dataset}}       & \multirow{2}{*}{\textbf{Metrics}} & \multicolumn{3}{c|}{\textbf{RMG}}                & \multicolumn{3}{c}{\textbf{LEMON}}               \\
                                                    &                                   & \textbf{TF-TH} & \textbf{TF-CK} & \textbf{TH-CK} & \textbf{TF-TH} & \textbf{TF-CK} & \textbf{TH-CK} \\ \midrule
            \multirow{3}{*}{\textbf{CIFAR-10}}      & \textbf{FC}                       & 1              & 1              & 0              & 1              & 1              & 0              \\
                                                    & \textbf{LC}                       & 0              & 0              & 1              & -              & -              & -              \\
                                                    & \textbf{BC}                       & 0              & 0              & 5              & -              & -              & -              \\ \midrule
            \multirow{3}{*}{\textbf{MNIST}}         & \textbf{FC}                       & 0              & 0              & 0              & 0              & 0              & 0              \\
                                                    & \textbf{LC}                       & 1              & 0              & 1              & -              & -              & -              \\
                                                    & \textbf{BC}                       & 0              & 0              & 0              & -              & -              & -              \\ \midrule
            \multirow{3}{*}{\textbf{F-MNIST}} & \textbf{FC}                       & 1              & 0              & 1              & 1              & 0              & 1              \\
                                                    & \textbf{LC}                       & 0              & 2              & 0              & -              & -              & -              \\
                                                    & \textbf{BC}                       & 0              & 2              & 0              & -              & -              & -              \\ \midrule
            \multirow{3}{*}{\textbf{ImageNet}}      & \textbf{FC}                       & 0              & 0              & 0                & 1              & 1              & 0              \\
                                                    & \textbf{LC}                       & 0               & 0               & 0               & -              & -              & -              \\
                                                    & \textbf{BC}                       & 1               & 2               & 2               & -              & -              & -              \\ \midrule
            \multirow{3}{*}{\textbf{Sine-Wave}}     & \textbf{FC}                       & 0              & 1              & 1              & 0              & 1              & 1              \\
                                                    & \textbf{LC}                       & 0              & 0              & 0              & -              & -              & -              \\
                                                    & \textbf{BC}                       & 0              & 0              & 0              & -              & -              & -              \\ \midrule
            \multirow{3}{*}{\textbf{Stock-Price}}   & \textbf{FC}                       & 0              & 0              & 0              & 0              & 0              & 0              \\
                                                    & \textbf{LC}                       & 0              & 0              & 0              & -              & -              & -              \\
                                                    & \textbf{BC}                       & 0              & 0              & 0              & -              & -              & -              \\ \bottomrule
        \end{tabular}

        % % 表格注释
        % \begin{tablenotes}
        %     \footnotesize
        %     \item[1] XXX
        % \end{tablenotes}

    \end{threeparttable}
    }
    \label{table:run_lemon_models}
\end{table}

